Multi-Agent Feedback Motion Planning using Probably Approximately Correct Nonlinear Model Predictive Control

For many tasks, multi-robot teams often provide greater efficiency, robustness, and resiliency. However, multi-robot collaboration in real-world scenarios poses a number of major challenges, especially when dynamic robots must balance competing objectives like formation control and obstacle avoidance in the presence of stochastic dynamics and sensor uncertainty. In this paper, we propose a distributed, multi-agent receding-horizon feedback motion planning approach using Probably Approximately Correct Nonlinear Model Predictive Control (PAC-NMPC) that is able to reason about both model and measurement uncertainty to achieve robust multi-agent formation control while navigating cluttered obstacle fields and avoiding inter-robot collisions. Our approach relies not only on the underlying PAC-NMPC algorithm but also on a terminal cost-function derived from gyroscopic obstacle avoidance. Through numerical simulation, we show that our distributed approach performs on par with a centralized formulation, that it offers improved performance in the case of significant measurement noise, and that it can scale to more complex dynamical systems.

==> approach.tex <==
\section{Approach}
\subsection{Problem Formulation}
The objective is to navigate a team of robots through an obstacle field from a set of initial states $x_I$ to a set of goal states $x_G$ while maintaining a formation. 

We apply a PAC-NMPC to each agent separately. The agents travel in a formation based on a leader-follower approach. The leader agent plans a trajectory based on a global goal state $x_G$. The followers plan their trajectories based on a state calculated using the leader state $x_L$, which can be any function that depends on the leader's state.

\subsection{Multi-Agent Collision Constraints}

The PAC-NMPC approach can plan to avoid static obstacles and could be modified for non-accelerating obstacles. However, an agent constraint must be defined since the other agents are accelerating and constantly re-planning their trajectories. 

Since each agent is optimizing a control policy at each planning step, each agent will share their control policy and state after each planning cycle. 

\begin{algorithm}
\caption{Agent Policy Optimization}
\begin{algorithmic}
\State Receive Agents states and policies
\State Sample Other Agent Trajectories
\While {termination conditions not met}
    \For{$j = 1,2,...,M$}
        \State Sample Trajectory: $(\tau_j,\xi_j) \gets p(\cdot ,\cdot | \hat{\nu}_0^*));$
        \State Evaluate Cost $J_j = J(\tau_j)$;
        \State Evaluate Constraint $C_j = C(\tau_j)$
    \EndFor
    \State $\hat{\nu}_{i+1}^* = argmin_{\nu} \hat{J}(\nu) + \alpha D(\nu,\hat{\nu}_i^*);$
\EndWhile
\state Share State and Policy
\end{algorithmic}
\end{algorithm}

When each agent $i$ starts its trajectory planning interval, it samples trajectories for every other agent $j$ in its team, using agent $j$'s control policy and states. This gives agent $i$ a set of guessed trajectories for all the other agents. When agent $i$ starts to optimize its trajectories, it uses the guessed trajectories for all other agents and treats those trajectory points at each time step as obstacles.

\begin{algorithm}
\caption{Sample Other Agents' Trajectories}
\begin{algorithmic}
\For{$a = 1,2,...,N_A$} \Comment{$N_A$ is the number of Agents}
    \If {$a \neq A$} 
    \For{$j = 1,2,...,M$}
            \State Sample Trajectory: $(\tau_{a,j},\xi_{a,j}) \gets p_a(\cdot ,\cdot | \hat{\nu}_0^*));$
            \Comment{Save trajectories for each agent}
    \EndFor
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Interagent Collision Avoidance Constraint $i$}
\begin{algorithmic}
\For{$j = 1,...,M$} \Comment{Iterate through trajectories}
    \For{$t = 1,...,N_t$} \Comment{all time steps}
        \For{$a = 1,2,...,N_A$}  \Comment{All agents}
            \State $\bx_a \gets Sample(a,j,t)$ \Comment{get predicted state}
            \State $\bold{dx} \gets \bx_i - \bx_a$
            \If{$||dx|| < L^2$}
                \State return \textbf{1}
           \EndIf 
        \EndFor
    \EndFor
\EndFor
\State return \textbf{0}
\end{algorithmic}
\end{algorithm}



\subsection{State Estimation Error}

The distributed approach requires information about each agent to be sent to all other agents to avoid collisions. However, having the ground truth about an environment is only possible in simulation. We simulate noise in state estimation by adding a zero mean noise to the sent-out state. When the agent receives the state of another agent, it also gets the state's variance (i.e., provided by a state estimator such as a Kalman Filter). The state with noise is defined as

\begin{align}
    x_{i,error} \sim N(x_i,\sigma_i^2),
\end{align}

where $x_i$ is the ground truth state, $x_{i,error}$ is the received agent state and $\sigma_i$ is that state variable's variance.

The algorithm accounts for the noise in the other agents' states by sampling a state from the received distribution for the agent when rolling out sample trajectories. The sampled state is pulled from a Gaussian distribution with a mean and variance of the received state and variance for that agent. 

\begin{algorithm}
    \caption{Noisy State Trajectory Sample}
    \begin{algorithmic}
        \For{$j = 1,2,...,M$}
            \State $\bx_{j,0} \gets p(x_0,\sigma)$
            \State Sample Trajectory: $(\tau_j,\xi_{j,0}) \gets p(\cdot ,\cdot | \hat{\nu}_0^*));$
        \EndFor
    \end{algorithmic}
\end{algorithm}



\subsection{Cost Functions}

For the formation control, we are using a Leader-Follower approach.
Since the goal states for the follower agents are based on the leader's state, the follower goal states can and will change rapidly throughout the plan. 

We defined a velocity field that accounted for the obstacle field near the agent. This approach gives a vector at each point in space that is the sum of the go-to vector and obstacle avoidance vector \cite{BRAQUET2022587}. After creating this velocity field, our new cost function becomes 
\begin{align}
    J(\bX) = \omega_1||(velocityField(x,x_G) - v)|| + \omega_2||x-x_d||
\end{align}
where $v$ is the agent's velocity at the end of the trajectory, $x$ is the agent's position, and $x_d$ is the agent's desired position.

\begin{algorithm}
    \caption{Velocity Field (state, goal)} 
    \begin{algorithmic}
        \State Initialize the velocity field $velocityField \gets 0$
        \For {each obstacle in the environment}
            \State  $angleToGoal = \arctan(\frac{obstacleY-goalY}{obstacleX-goalX})$ 
            \State  $distanceToObstacle = |state-obstacle| - r$
            \State  $rotationMatrix = Rot(angleToGoal)$ 
            \If {$distanceToObstacle < detectionRange \And distanceToObstacle > 0 $} 
                \State  $angleToObstacle =  \arctan(\frac{stateX - obstacleY}{stateY - obstacleX})$ 
                \State  $directionVector = [sin(angleToObstacle);cos(angleToObstacle)]$
                \State  $rotatedPosition = rotationMatrix*(state - obstacle)$
                \If {$rotatedPosition(1) < 0$} \Comment{Make the Vector Point Towards the Goal}
                    \State Reverse the direction $directionVector = -directionVector$
                \EndIf
                \If {$rotatedPosition(0) < -0.5*r$} 
                    \State  $directionVector = 0*directionVector$ 
                \EndIf
                \State  $velocityField = velocityField + directionVector/distanceToObstacle$ 
            \EndIf
        \EndFor
  \end{algorithmic}
\end{algorithm}


\subsection{Formation Goal Points in Obstacle Fields}
When the formation is in an obstacle field, we adjust the formation to keep the followers from having a goal in an obstacle. For this, we pull the formation goal point closer to the leader if the goal is an obstacle. We define the move as follows:
\begin{align}
x_G^{i} &= x_{obs} + (r_{obs}^i/d)*(x_{obs}^i - \Bar{x_i}) \nonumber\\ .
\end{align}
Where $x_G^{i}$ is the goal for agent $i$, $x_{obs}$ and $r_{obs}^i$ are the x and y coordinates and radius of obstacle $i$ respectively, $d$ is the distance between the obstacle and the leader agent, and $\Bar{x_i}$ is the position of agent $i$.


